Quantum Extremal Islands Made Easy, Part IV: Massive Black Holes on the Brane

We study two-dimensional eternal black holes with non-zero mass, where each asymptotic boundary is in contact with a CFT on a circle, following the doubly holographic braneworld models constructed in [arXiv:2006.04851, arXiv:2010.00018, arXiv:2010.16398]. We compute the Page curve of the black hole (or the bath CFTs), which amounts to finding different geodesics in the bulk BTZ geometry with a Randall-Sundrum brane falling into the black hole. We also explore the possibility of including an intrinsic JT gravity action on the brane. As expected, the generalized entropy rises linearly at early times. However, there is a transition to a late-time phase in which the entropy remains constant. The value of the late-time entropy depends on the size of the thermal baths. For a small size, it corresponds to the thermal entropy of the baths, while for large size, it corresponds to twice the horizon entropy of the black hole. The critical size and the Page time are proportional to ratio of the central charges of the conformal defect and the bath CFT.

==> sections/setup.tex <==
% !TEX root = ../QEIv02.tex

\rcm{Drop this section. Fold important bits into next section.}
\subsection{The braneworld framework} \label{sec:2.4}
\begin{figure}
	\centering
	\includegraphics[scale = 0.7]{figures/randall_sundrum.png}
	\caption{Time slice for the construction of the bulk geometry with a Randall-Sundrum brane. In (a) the bulk space is cut off at some co-dimension one AdS slice, and in (b) the remaining space is glued to another copy of itself along the cut, which takes the role of the brane. Figure taken from \cite{partii}.}
	\label{fig:randallsundrum}
\end{figure}
In this section, we will review the geometric setup introduced in \cite{parti, partii}. We start with our bulk gravitational theory, which is Einstein gravity in $(d+1)$ dimensions
\begin{equation}
I_{\text{bulk}} = \frac{1}{16\pi G_{\text{bulk}}}\int \dd^{d+1}x\sqrt{-g}\left[R + \frac{d(d-1)}{L^2}\right]
\end{equation}
where $G_{\text{bulk}}$ is the $(d+1)-$dimensional Newton constant, $L$ is the AdS scale and $g_{ab}$ is the metric in the bulk. Furthermore, we introduce a $d-$dimensional brane in the bulk with action\footnote{One can further add an intrinsic Einstein-Hilbert term for the Ricci scalar $R(h)$ on the brane. This term is natural if we want to generalize JT gravity for the case of $d = 2$. More about it in section \ref{sec:chapter4}.}
\begin{equation}\label{eq:braneaction}
I_{\text{brane}} = - T_0 \int \dd^d x \sqrt{-h}
\end{equation}
where $h_{ab}$ is the induced metric on the brane and $T_0$ is the tension of the brane. The brane is taken to have an induced geometry\footnote{This can be justified by a symmetry consideration. In usual AdS/CFT, the duality between conformal field theories and Anti de Sitter spacetimes is justified (at least at an intuitive explanation) by the two having the same symmetry structure. The conformal group of the CFT in $d$ dimensions is $\text{SO(d,2)}$, which is the same as the isometry group of $(d+1)-$dimensional Anti de Sitter space. Likewise, the conformal symmetry on the defect is SO($d-1$,2) and so one expects the same symmetry on the brane, thus having $d-$dimensional AdS geometry on it.} that is locally AdS and so one can consider the foliation of $\text{AdS}_{d+1}$ in $\text{AdS}_{d}$ unit-curvature slices as follows
\begin{equation}
\dd{s}_{\text{AdS}_{d+1}}^2 = \frac{L^2}{\sin^2{\theta}}(\dd{\theta}^2 + \dd{s}_{\text{AdS}_{d}}^2)
\end{equation}
where $0\leq \theta \leq \pi$. To construct the brane we follow the Randall-Karch models \cite{KarchRandall1, KarchRandall2}, where one cuts the spacetime along one of the AdS slices near the asymptotic boundary $\theta = 0$, at some $\theta_B \ll 1$.\footnote{This corresponds to the brane having a large tension.} Then, one takes an exact copy of this spacetime and glues the two together: the brane appears along the gluing of the two boundaries. The two geometries have the metric as given above for $\theta_B \leq \theta \leq \pi$. Furthermore, while the brane splits the spacetime in half, each half is more than half of empty AdS due to the brane's backreaction which enlarges the geometry. This backreaction induces an effective theory of dynamical Einstein gravity on the brane. We will postpone the effective gravity description to section \ref{sec:3.4}, focusing now on the bulk description. How do we find the brane position $\theta_B$? This is dictated by the Israel junction conditions \cite{Israel} which fix $\theta_B$ by associating the jump in the extrinsic curvature $K_{ij}$ across the brane to its tension \cite{parti,partii}, as follows. The variation of the bulk action $I_{\text{bulk}} + I_{\text{brane}}$ w.r.t the induced metric $h_{ij}$ imposes the following condition \cite{Israel}
\begin{equation}
\Delta K_{ij} - h_{ij} \Delta K^{i}_{\;\;i} = 8\pi G S_{ij}
\end{equation}
where $S_{ij}$ is the energy momentum tensor induced on the brane and $\Delta K_{ij} = 2K_{ij}$ is the discontinuity of the extrinsic curvature across the hypersurface. Since $S_{ij} = -T_0 h_{ij}$, the junction condition becomes
\begin{equation}\label{eq:junction}
K_{ij} = \frac{4\pi G T_0}{d-1} h_{ij}.
\end{equation}
Using the above, one finds \cite{parti, partii}
\begin{equation}\label{eq:braneprofile}
\sin^2{\theta_B} = \frac{L^2}{\ell_B^2} = 2\epsilon(1 - \epsilon/2), \;\;\;\; \epsilon \equiv \left(1 - \frac{4\pi G_{\text{bulk}} L T_0}{d-1}\right).
\end{equation}
where $\ell_B$ is the curvature scale on the brane. To sum up, the brane's position $\theta_{B}$ is determined through the above procedure in terms of the brane's tension. The bulk picture is now complete, and its the dual picture to the boundary perspective: where we have a CFT living on a cylinder $\mathbb{R} \times S^{d-1}$ with a $(d-1)-$dimensional defect positioned at the equator.

\subsection{The case of two dimensions}\label{sec:2.5}
\begin{figure}
	\centering
	\includegraphics[scale = 0.6]{figures/rindlerbrane.pdf}
	\caption{Penrose diagram in the brane perspective of the doubly holographic model of a black hole in thermal equilibrium with an external bath. In purple and yellow we have the two bath CFT regions, each coupled with an AdS topological black hole at the defect (showed in dark green). The drawing is also valid in dimensions $d>2$, where each point represents an hyperbolic space $H_{d-2}$. Image recreated from \cite{partii}.}
	\label{fig:rindlerbrane}
\end{figure}
Let us review the case of having three-dimensional gravity in the bulk with a two-dimensional brane since it will be the case we will do the computations in the next section. To study eternal black holes on the brane, the authors of \cite{partii} conveniently chose to use AdS-Rindler coordinates
\begin{equation}\label{eq:BH0}
\dd{s}^2 = L^2\left[(r^2- 1)\dd{t}^2 + \frac{\dd{r}^2}{r^2 - 1} + r^2 \dd{\chi}^2\right]
\end{equation}
where $\chi \in \mathbb{R}$. Writing pure AdS in these coordinates allows to view it as a topological massless black hole with an apparent horizon at $r = 1$ and a coordinate singularity at $r = 0$. It is possible to show that the brane also inherits an AdS-Rindler geometry \cite{partii}, with metric
\begin{equation}
\dd{s}^2 = \ell_B^2\left[-(\rho^2 -1)\dd{t}^2 + \frac{\dd\rho^2}{\rho -1}\right].
\end{equation}
where $\ell_B^2(\rho^2 - 1) = L^2(r^2 - 1)$. In the brane perspective, we have a CFT living on the two Rindler boundaries and on the Rindler-$\text{AdS}_2$ black hole. With a $\mathbb{Z}_2$ across the brane, this doubly holographic model becomes essentially the model considered in \cite{almheiri2019eternal}. The brane perspective of this geometry is shown in fig. \ref{fig:rindlerbrane}. One can then compute entanglement entropies for subregions in the baths CFT using the entanglement entropy formula introduced before. One finds two competing phases which exchange dominance at some time $t_P$: the Page time. The two phases differ by the formation of islands. Because the black hole is eternal, after the Page time, the growth stops and the entropy saturates. A Page curve is thus recovered for such an holographic system of topological black holes coupled to a thermal bath. We will now repeat the same idea, but with massive black holes. 
